Effectively Unbiased FID and Inception Score and where to find them

This paper shows that two commonly used evaluation metrics for generative models, the Fr\'echet Inception Distance (FID) and the Inception Score (IS), are biased -- the expected value of the score computed for a finite sample set is not the true value of the score. Worse, the paper shows that the bias term depends on the particular model being evaluated, so model A may get a better score than model B simply because model A's bias term is smaller. This effect cannot be fixed by evaluating at a fixed number of samples. This means all comparisons using FID or IS as currently computed are unreliable. We then show how to extrapolate the score to obtain an effectively bias-free estimate of scores computed with an infinite number of samples, which we term $\overline{\textrm{FID}}_\infty$ and $\overline{\textrm{IS}}_\infty$. In turn, this effectively bias-free estimate requires good estimates of scores with a finite number of samples. We show that using Quasi-Monte Carlo integration notably improves estimates of FID and IS for finite sample sets. Our extrapolated scores are simple, drop-in replacements for the finite sample scores. Additionally, we show that using low discrepancy sequence in GAN training offers small improvements in the resulting generator.

==> FID infinity arxiv/algorithm.tex <==
\begin{algorithm}
\caption{Evaluating $\overline{\textrm{FID}}_\infty$ for a Generator }
\begin{algorithmic}[1]
\State $G$: Generator
\State $I$: Inception Network
\State $n$: Number of images we want to generate
\State $t$: Number of FIDs we compute for extrapolation
\State $m_t$: Precomputed groundtruth activations mean
\State $c_t$: Precomputed groundtruth activations covariance 
\State 
\Procedure{Evaluate}{$G, I, n, t, m_t, c_t$}
    \State FID $= \{\}$
    \State $z \gets \textsc{SobolSampler($n$)}$
    \State activations $\gets I(G(z))$
    \State
    \LineComment $5000$ is the min no. of images we evaluate with
    \State batchSizes = $\textsc{linspace($5000, n, t)$}$
    \For{batchSize in batchSizes}
        \State \textsc{Shuffle(\textnormal{activations})}
        \State activations$_i$ $\gets$ activations[:batchSize]
        \State FID.insert(\textsc{CalculateFID(\textnormal{activations$_i$, $m_t, c_t$})})
    \EndFor
    \State reg $\gets \textsc{LinearRegression(1/\textnormal{batchSizes, FID})}$
    \State $\overline{\textrm{FID}}_\infty \gets$ reg.predict($0$)
    \State \textbf{return} $\overline{\textrm{FID}}_\infty$
\EndProcedure
\end{algorithmic}
\end{algorithm}


==> FID infinity arxiv/figures/IS_error.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.55]{figures/IS_error_fig.pdf}
    \caption{IS$_{100\textrm{k}}$ predictions using $50$k images are highly accurate with low variance. The figure shows error plots of $\overline{\textrm{IS}}_{100\textrm{k}}$ for BigGAN trained on ImageNet and CIFAR10 over $50$ runs. Sobol$_{Inv}$ gives the best accuracy with low standard deviations. The plots follow the same markings as Figure \ref{fig:error_plot}.
    }
    \label{fig:IS_error}
\end{figure}


==> FID infinity arxiv/figures/IS_graph.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.4]{figures/IS_graph_fig.pdf}
    \caption{IS$_N$ is negatively biased. IS$_N$ vs $\frac{1}{N}$ of BigGAN for $3$ sampling methods where each point is an average over (a): $1$ split, (b): $50$ splits. For (b), error bars represent standard deviation and the line joins the IS$_N$ estimates mean of Sobol$_{Inv}$. Unlike FID$_N$, IS$_N$ increases with increasing $N$, suggesting negative bias. From (b) the variance of IS$_N$ estimates from normal points are considerably higher than those of Sobol sequences, which is also evidenced by Table~\ref{tbl:fid_tables}. Figure (b) is best viewed in color and high resolution.}
    \label{fig:IS_graph}
\end{figure}


==> FID infinity arxiv/figures/compare_fid.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.6]{figures/compare_fid_fig.pdf}
    \caption{
        The choice of $N$ used affects comparison severely. The graph compares the FID$_N$ vs $\frac{1}{N}$ between two independently trained identical architecture DCGANs. At marker $1$, DCGAN 1 is better than DCGAN 2; at marker 2 they are approximately the same; at marker 3 DCGAN 2 is better than DCGAN 1. This shows that comparisons between models of a fixed $N$ are unreliable.
    }
    \label{fig:compare_fid}
\end{figure}


==> FID infinity arxiv/figures/error_plot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.55]{figures/error_plot_fig.pdf}
    \caption{
        FID$_{100\textrm{k}}$ predictions are highly accurate compared to groundtruth (horizontal line) with low variance using $50$k images. This suggests predicting FID$_\infty$ is sound. The figure shows error plots of $\overline{\textrm{FID}}_{100\textrm{k}}$ with $y$ axis of the same scale. The point represent the mean, and the error bar the standard deviation over $50$ runs. The far left point is the target FID$_{100\textrm{k}}$ we are estimating. For each sampling method, we estimate FID$_{100\textrm{k}}$ by fitting points over regular intervals over $N$ (dots) or over $\frac{1}{N}$ intervals (triangles). We also color-tagged the lowest 3 standard deviations. Overall, Sobol$_{Inv}$ with intervals over $N$ perform the best, with good accuracy and low variance. Best viewed in color and high resolution.
    }
    \label{fig:error_plot}
\end{figure}


==> FID infinity arxiv/figures/fid_infinity.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.55]{figures/fid_infinity_fig.pdf}
    \caption{Error plots of predicting FID$_\infty$ over $50$ runs. $\overline{\textrm{FID}}_\infty$ have low variance and are consistent. This together with Figure~\ref{fig:error_plot} suggests that they are accurate. The plots follow the same markings as Figure \ref{fig:error_plot}.
    }
    \label{fig:fid_infinity}
\end{figure}


==> FID infinity arxiv/figures/graph.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.7]{figures/graph_fig.pdf}
    \caption{2d scatter plots of $1000$ random points vs Sobol and Scrambled Sobol points. Sobol sequences give us evenly spaced samples while random sampling results in clusters and empty spaces due to their IID property.}
    \label{fig:graph}
\end{figure}


==> FID infinity arxiv/figures/linear_fid.tex <==
\begin{figure}[t]
    \centering
    %\hspace*{-1cm}
    \includegraphics[scale = 0.5]{figures/linear_fid_fig.pdf}
    \caption{
        Plots of FID vs $\frac{1}{N}$ for various models with various sampling methods at the same scale. Each FID point corresponds to a single FID estimate. FIDs are linear with respect to $\frac{1}{N}$ across all experiments, with higher variance (more spikes) when $N$ is small. Most importantly, the slopes, which corresponds to the $K$ term of eq \ref{eq:linear_fid}, are very different across models. Even though the models are not directly comparable since they generate different datasets, this shows different models have very different $K$ terms. Comparisons of different models with FID$_N$ at fixed $N$ are unreliable because they are dominated by bias.}
    \label{fig:linear_fid}
\end{figure}    



==> FID infinity arxiv/figures/predict_plot.tex <==
\begin{figure}[t]
    \centering
    \hspace*{-.6cm}
    \includegraphics[scale = 0.6]{figures/predict_plot_fig.pdf}
    \caption{
        FID$_N$ estimates give very good line fits, especially with Sobol$_{Inv}$ (right), suggesting extrapolation will succeed (it does, see Fig \ref{fig:error_plot}). The figure shows the line fits for predicting FID$_{100\textrm{k}}$ for a random DCGAN. Green point is the target FID$_{100\textrm{k}}$ while the blue crosses are the FIDs we compute to fit a linear regression. The columns represents the sampler we use to generate images while the rows represent how we choose $N$ to compute FID. \textbf{Row 1:} choose at regular intervals over $N$; \textbf{Row 2:} choose at regular intervals over $\frac{1}{N}$. For the normal sampler, there are more outliers and the prediction is not as accurate. Using Sobol$_{Inv}$ and computing FIDs at regular intervals over $N$ (Figure \textbf{(b)}) give us better line fit for predicting FID$_{100\textrm{k}}$.}
    \label{fig:predict_plot}
\end{figure}


==> FID infinity arxiv/figures/train_gan.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.6]{figures/train_gan_fig.pdf}
    \caption{Training GANs with Sobol sequence results in better or comparable $\overline{\textrm{FID}}_\infty$ and lower variance between training runs. The figures show sorted $\overline{\textrm{FID}}_\infty$ of $12$ GANs trained with different sampling methods for two resolutions of CelebA. Each $\overline{\textrm{FID}}_\infty$ is an average of $50$ calculations.}
    \label{fig:train_gan}
\end{figure}


==> FID infinity arxiv/figures/vae.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[scale = 0.7]{figures/vae_fig.pdf}
    \caption{Error plots of predicting FID$_\infty$ for a VAE over $50$ runs. $\overline{\textrm{FID}}_\infty$ works regardless for model used, in this case for VAE. The plots follow the same markings as Figure \ref{fig:error_plot}.
    }
    \label{fig:vae}
\end{figure}


==> FID infinity arxiv/sobol_code.tex <==
\begin{lstlisting}[language=Python, caption=PyTorch code for generating Sobol points, float=*]
from botorch.sampling.qmc import NormalQMCEngine

class randn_sampler():
    """
    Generates z~N(0,1) using random sampling or scrambled Sobol sequences.
    Args:
        ndim: (int)
            The dimension of z.
        use_sobol: (bool)
            If True, sample z from scrambled Sobol sequence. Else, sample 
            from standard normal distribution.
            Default: False
        use_inv: (bool)
            If True, use inverse CDF to transform z from U[0,1] to N(0,1).
            Else, use Box-Muller transformation.
            Default: True
        cache: (bool)
            If True, we cache some amount of Sobol points and reorder them.
            This is mainly used for training GANs when we use two separate
            Sobol generators which helps stabilize the training.
            Default: False
            
    Examples::

        >>> sampler = randn_sampler(128, True)
        >>> z = sampler.draw(10) # Generates [10, 128] vector
    """

    def __init__(self, ndim, use_sobol=False, use_inv=True, cache=False):
        self.ndim = ndim
        self.cache = cache
        if use_sobol:
            self.sampler = NormalQMCEngine(d=ndim, inv_transform=use_inv)
            self.cached_points = torch.tensor([])
        else:
            self.sampler = None

    def draw(self, batch_size):
        if self.sampler is None:
            return torch.randn([batch_size, self.ndim])
        else:
            if self.cache:
                if len(self.cached_points) < batch_size:
                    # sample from sampler and reorder the points
                    self.cached_points = self.sampler.draw(int(1e6))[torch.randperm(int(1e6))]

                # Sample without replacement from cached points
                samples = self.cached_points[:batch_size]
                self.cached_points = self.cached_points[batch_size:]
                return samples
            else:
                return self.sampler.draw(batch_size)
\end{lstlisting}


==> FID infinity arxiv/tables/extrapolate.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\cline{5-7}
      & \multicolumn{3}{c}{DCGAN}                         & \multicolumn{3}{c|}{ProGAN}                      \\ \cline{5-7} 
      & Actual          & Sobol (BM)     & Sobol (Inv)    & Actual         & Sobol (BM)     & Sobol (Inv)    \\ \cline{5-5}
10000 & 15.67 +- 0.098  & 15.30 +- 0.181 & 15.40 +- 0.197 & 10.98 +- 0.082 & 10.84 +- 0.172 & 10.80 +- 0.168 \\ \cline{5-5}
25000 & 14.86 +- 0.083  & 14.38 +- 0.273 & 14.43 +- 0.244 & 10.20 +- 0.048 & 10.01 +- 0.195 & 9.95 +- 0.229  \\ \cline{5-5}
50000 & 14.57  +- 0.046 & 14.24 +- 0.280 & 14.21 +- 0.213 & 9.94 +- 0.045  & 9.70 +- 0.178  & 9.68 +- 0.158  \\ \cline{5-5}
\end{tabular}%
}
\caption{We use only $5000$ generated images to predict the FID scores of different models when evaluated with different number of images. The predicted FID scores are close to the actual FID score but biased lower.}
\label{tbl:extrapolate}
\end{table*}


==> FID infinity arxiv/tables/fid_tables.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|c|c|c|c|c|c|c}
                 & \multicolumn{2}{c}{Normal}                              & \multicolumn{3}{c}{{\color[HTML]{333333} Sobol$_{BM}$}}                                                           & \multicolumn{3}{c}{Sobol$_{Inv}$}                                   \\\hline
Models           & \cellcolor[HTML]{C0C0C0}FID$_{50\textrm{k}}$             & IS$_{5\textrm{k}}$             & \cellcolor[HTML]{C0C0C0} FID$_{50\textrm{k}}$         &  IS$_{5\textrm{k}}$            & F Value & \cellcolor[HTML]{C0C0C0}FID$_{50\textrm{k}}$             & IS$_{5\textrm{k}}$             & F Value \\\hline
DCGAN          & \cellcolor[HTML]{C0C0C0}14.61 $\pm$ 0.0579 & -              & \cellcolor[HTML]{C0C0C0} 14.59 $\pm$ 0.0471 &  -              & 1.51    & \cellcolor[HTML]{C0C0C0}\textbf{14.58 $\pm$ 0.0439} & -              & 1.74    \\
ProGAN           & \cellcolor[HTML]{C0C0C0}9.94 $\pm$ 0.0411  & -              & \cellcolor[HTML]{C0C0C0} \textbf{9.94 $\pm$ 0.0384}  & -              & 1.14    & \cellcolor[HTML]{C0C0C0}9.94 $\pm$ 0.0404  & -              & 1.03    \\
StyleGAN         & \cellcolor[HTML]{C0C0C0}4.33 $\pm$ 0.0413  & -              & \cellcolor[HTML]{C0C0C0} 4.33 $\pm$ 0.0406  &  -              & 1.03    & \cellcolor[HTML]{C0C0C0}\textbf{4.33 $\pm$ 0.0354}  & -              & 1.36    \\\hline
    BigGAN           & \cellcolor[HTML]{C0C0C0}9.94 $\pm$ 0.0564  & 92.96 $\pm$ 2.135 & \cellcolor[HTML]{C0C0C0} \textbf{9.92} $\pm$ 0.0576  & 92.89 $\pm$ 1.961 & 1.19    & \cellcolor[HTML]{C0C0C0}9.93 $\pm$ \textbf{0.0419}  & \textbf{93.21 $\pm$ 1.640} & 1.69    \\
    BigGAN (CIFAR10) & \cellcolor[HTML]{C0C0C0}8.26 $\pm$ 0.0467  & 8.44 $\pm$ 0.1223 & \cellcolor[HTML]{C0C0C0}  \textbf{8.25} $\pm$ 0.0455  & \textbf{8.48} $\pm$ 0.1172 & 1.09    & \cellcolor[HTML]{C0C0C0}8.26 $\pm$  \textbf{0.0446} & 8.45 $\pm$ \textbf{0.1018} & 1.44   
\end{tabular}%
}
\caption{
Using Sobol sequences always give better FID and Inception Score (IS) along with lower standard deviations. The table shows FID$_{50\textrm{k}}$ (lower better) and IS$_{5\textrm{k}}$ (higher better) values of different models evaluated on Normal and Sobol sequences over $50$ runs. The F value is the ratio between the variances of the Normal and Sobol Sequences (the higher it is, the more different their variances are). Bolded values indicate the best score or standard deviation. Better scores implies lower bias which implies lower integrator variance.}
\label{tbl:fid_tables}
\end{table*}


==> tables/extrapolate.tex <==
\begin{table*}[t]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|ccc|ccc}
\cline{5-7}
      & \multicolumn{3}{c}{DCGAN}                         & \multicolumn{3}{c|}{ProGAN}                      \\ \cline{5-7} 
      & Actual          & Sobol (BM)     & Sobol (Inv)    & Actual         & Sobol (BM)     & Sobol (Inv)    \\ \cline{5-5}
10000 & 15.67 +- 0.098  & 15.30 +- 0.181 & 15.40 +- 0.197 & 10.98 +- 0.082 & 10.84 +- 0.172 & 10.80 +- 0.168 \\ \cline{5-5}
25000 & 14.86 +- 0.083  & 14.38 +- 0.273 & 14.43 +- 0.244 & 10.20 +- 0.048 & 10.01 +- 0.195 & 9.95 +- 0.229  \\ \cline{5-5}
50000 & 14.57  +- 0.046 & 14.24 +- 0.280 & 14.21 +- 0.213 & 9.94 +- 0.045  & 9.70 +- 0.178  & 9.68 +- 0.158  \\ \cline{5-5}
\end{tabular}%
}
\caption{We use only $5000$ generated images to predict the FID scores of different models when evaluated with different number of images. The predicted FID scores are close to the actual FID score but biased lower.}
\label{tbl:extrapolate}
\end{table*}

